Can we predict the Most Replayed data of video streaming platforms?

Predicting which specific parts of a video users will replay is important for several applications, including targeted advertisement placement on video platforms and assisting video creators. In this work, we explore whether it is possible to predict the Most Replayed (MR) data from YouTube videos. To this end, we curate a large video benchmark, the YTMR500 dataset, which comprises 500 YouTube videos with MR data annotations. We evaluate Deep Learning (DL) models of varying complexity on our dataset and perform an extensive ablation study. In addition, we conduct a user study to estimate the human performance on MR data prediction. Our results show that, although by a narrow margin, all the evaluated DL models outperform random predictions. Additionally, they exceed human-level accuracy. This suggests that predicting the MR data is a difficult task that can be enhanced through the assistance of DL. Finally, we believe that DL performance on MR data prediction can be further improved, for example, by using multi-modal learning. We encourage the research community to use our benchmark dataset to further investigate automatic MR data prediction.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> model-linear_planar.tex <==
\begin{tikzpicture}[font=\sffamily,module/.style={draw, very thick, rounded corners, minimum width=15ex},
smallmodule/.style={draw, very thick, rounded corners, minimum width=5ex},
embmodule/.style={module, fill=red!20},
segmodule/.style={smallmodule, fill=red!20},
gamodule/.style={module, fill=orange!20},
localmodule/.style={module, fill=orange!20},
mhamodule/.style={module, fill=orange!20},
lnmodule/.style={module, fill=yellow!20},
ffnmodule/.style={module, fill=cyan!20},
arrow/.style={-stealth, thick, rounded corners},
line/.style={thick, rounded corners},
]
\matrix [column sep=0cm, anchor=center] (feat) {
     \foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {
    \draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.275) -- (\x+0.075,0.3) -- (\x+0.075,-0.275) -- cycle;
      }; &
    \node[align=center] {$\dots$}; &
    \foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {
        \draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.275) -- (\x+0.075,0.3) -- (\x+0.075,-0.275) -- cycle;
    };\\
};
\node[left=0cm of feat] (i3dtext) {I3D features};
\begin{scope}[on background layer]
\node[fit={(feat)(i3dtext)}, embmodule, align=center] (i3d) {};
\end{scope}
\matrix [below=of i3d, column sep=0cm, anchor=center] (frames) {
 1 &
 \foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {
\draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.2) -- (\x+0.3,0.3) -- (\x+0.3,-0.2) -- cycle;
  }; &
\node[align=center] {$\dots$}; &
\foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {
    \draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.2) -- (\x+0.3,0.3) -- (\x+0.3,-0.2) -- cycle;
};\\
};
\node[left=0cm of frames] (inputstext) {Inputs};

% \matrix[above=1.7cm of i3d, column sep={0.05cm, 0cm, 0cm, 0.05cm}] (seg) {
% \foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {
%     \draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.275) -- (\x+0.075,0.3) -- (\x+0.075,-0.275) -- cycle;
%       }; &
%       \foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {
%     \draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.275) -- (\x+0.075,0.3) -- (\x+0.075,-0.275) -- cycle;
%       }; &
%       \node[align=center, text width=10px, anchor=center] {\small$\dots$}; &
%       \foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {    \draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.275) -- (\x+0.075,0.3) -- (\x+0.075,-0.275) -- cycle;
%       }; &
%       \foreach \n [evaluate=\n as \x using (\n)*0.15] in {0,...,2} {
%     \draw[fill=white!20,thick] (\x,-0.3) -- (\x+0.0,0.275) -- (\x+0.075,0.3) -- (\x+0.075,-0.275) -- cycle;
%       }; \\
%     % \node[segmodule, text width=0.52cm, minimum height=1cm] {}; &
%     % \node[segmodule, text width=0.52cm, minimum height=1cm] {}; &
%     % \node[segmodule, text width=0.52cm, minimum height=1cm] {}; &
%     % \node[segmodule, text width=0.52cm, minimum height=1cm] {}; \\
% };

\begin{scope}[on background layer]
\node[fit={(feat)(i3dtext)}, segmodule, align=center] (i3d) {};
\end{scope}

% \node[left=0cm of seg] (segtext) {Time windows};


% \matrix [above=2cm of seg, column sep=1cm,anchor=center] (local) {
%     \node[localmodule, text width=2cm, align=center] (local1) {Local Attention};  &
%     % label={[align=center]east:$1$st}
%     \node[align=center] {$\dots$}; &
%     \node[localmodule, text width=2cm, align=center] (localn) {Local Attention}; \\
%     % label={[align=center]east:$n$th}
%   };
% \node[above=of local, draw, thick, circle] (localplus) {$+$};
% \node[above=of localplus, draw, thick, circle] (plus) {$+$};

% \coordinate[right=5.5cm of plus] (residualhelper);
% \coordinate (segfork) at ($(seg.north)!0.5!(local.south)$);
% % \coordinate[below=1.5cm of seg] (arrowtip); % New coordinate for the arrowhead
% \coordinate (arrow1) at ($(i3d)!0.666!(seg)$); % Midpoint between i3d and seg
% \coordinate (arrow2) at ($(localplus)!0.333!(plus)$);
% \coordinate (arrowtip); % New coordinate for the arrowhead

% \coordinate (segfork) at ($(seg.north)!0.5!(local.south)$);


% \node[fit={(local)(localplus)(seg)(segtext)(arrow1)(arrow2)}, draw, dashed, thick, rounded corners] (localnode) {};

% \node[draw, thick, circle] (resplus) at (residualhelper) {$+$};
% \node[left=of local, gamodule, align=center] (ga) {Global\\Attention};
% \node[above=of local, lnmodule, align=center] (addnorm1) {Add \& Norm};
% \node[above=of addnorm1, ffnmodule, align=center] (ffn) {Feed\\Forward};
% \node[above=of ffn, lnmodule, align=center] (addnorm2) {Add \& Norm};
% \node[above=of addnorm2] (outputs) {Outputs};
% \node[left=of embplus, draw, thick, circle, inner sep=0pt,label={[align=left]left:Positional\\Encoding}] (pe) {\tikz \draw[scale=0.1] plot[domain=0.0:6.28] (\x,{sin(\x r)});};


\matrix[right=3cm of frames] (array) [matrix of math nodes, left delimiter={[}, right delimiter={]}] {
    \hat{y}_{1} & \hat{y}_{2} & \dots & \hat{y}_{I} \\
};
\node[left=0.25cm of array] (outputstext) {Output};

% \node[right=of resplus, yshift=-1cm, embmodule, align=center] (do1) {Dropout 0.5};
% \node[below=0.5cm of do1, lnmodule, align=center] (ln1) {LayerNorm};
\node[above=of array, ffnmodule, align=center] (fc2) {Linear Layer\\with Sigmoid};
\node[above=of fc2, lnmodule, align=center] (ln2) {LayerNorm};
\node[above=0.5cm of ln2, embmodule, align=center] (do2) {Dropout 0.5};
\node[above=of do2, ffnmodule, align=center] (fc1) {Linear Layer\\with ReLU};


\draw[arrow] (frames) -- (i3d);
% \draw[arrow] (localnode) -- (seg);
% \draw[arrow] (seg) -- (segfork);
% \draw[arrow] ([xshift=-1.1cm]seg.north) |- ([xshift=-1.5cm]segfork) -|  (local1);
% \draw[arrow] ([xshift=-0.6cm]seg.north) -- ([xshift=-0.6cm, yshift=1cm] seg.north);
% % \node[above=0cm of seg.north] (segdots) {$\dots$};
% % --  ([xshift=-0.5cm, yshift=0.8cm]segfork);
% \draw[arrow] ([xshift=0.6cm] seg.north) -- ([xshift=0.6cm, yshift=1cm] seg.north); 
% % -- ([xshift=0.5cm, yshift=0.8cm]segfork);
% \draw[arrow] ([xshift=1.1cm]seg.north) |- ([xshift=1.5cm]segfork)   -| (localn);
% \draw[arrow] (plus) -- (resplus);
% \draw[arrow] (i3d) -- (seg);
% \draw[arrow,] (i3d) -| (ga);
% \draw[arrow] (localplus) -- (plus);
% \draw[arrow] (local1) |- (localplus);
% \draw[arrow] (localn) |- (localplus);
% \draw[arrow] (ga) |- (plus);
% \draw[arrow] (i3d) -| node[above,sloped,xshift=5cm]{Residual connection} (resplus);

\draw[arrow] (i3d) |- (fc1);
% \draw[arrow] (do1) -- (ln1);
% \draw[arrow] (ln1) -- (fc1);
\draw[arrow] (fc1) -- (do2); 
\draw[arrow] (do2) -- (ln2);
\draw[arrow] (ln2) -- (fc2);
\draw[arrow] (fc2) -- (array);


% \draw[arrow] (mha) -- (addnorm1);
% \draw[arrow] (addnorm1) -- (ffn);
% \draw[arrow] (ffn) -- (addnorm2);
% \draw[arrow] (addnorm2) -- (outputs);

% \coordinate (ffnresidual) at ($(ffn.south)!0.5!(addnorm1.north)$);
% \coordinate (mhafork) at ($(mha.south)!0.5!(mharesidual)$);
% \coordinate[left=of addnorm1] (ln1residualleft);
% \coordinate[left=of addnorm2] (ln2residualleft);

% \node[fit={(mha)(addnorm2)(mharesidual)(ln1residualleft)}, draw, ultra thick, rounded corners, label=left:$\mathrm{N\times}$] (encoder) {};

% \draw[arrow] (mharesidual)-|(ln1residualleft)--(addnorm1);
% \draw[arrow] (ffnresidual)-|(ln2residualleft)--(addnorm2);
% \draw[arrow] (mhafork)-|($(mha.south)!0.5!(mha.south west)$);
% \draw[arrow] (mhafork)-|($(mha.south)!0.5!(mha.south east)$);

\end{tikzpicture}

==> sections/abstract_old.tex <==
Predicting which specific parts of a video users will 
% find interesting and 
replay is important for several applications, including targeted advertisement placement on video platforms and assisting video creators.
In this work, we explore whether it is possible to predict the \emph{Most Replayed} (MR) data from YouTube videos. 
To this end, we curate a large video benchmark, the \emph{YTMR500} dataset, which comprises 500 YouTube videos with MR data annotations. 
We evaluate Deep Learning (DL) models of varying complexity on our dataset and perform an extensive ablation study. In addition, we conduct a user study to estimate the human performance on MR data prediction.
Our results show that, although by a narrow margin, all the evaluated DL models outperform random predictions. %, demonstrating the predictability of MR data. 
% What if we dropped this?
% demonstrating the predictability of MR data. 
% I changed my mind, let's remove it :D XDD
Additionally, they exceed human-level accuracy. This suggests that predicting the MR data is a difficult task that can be enhanced through the assistance of AI. 
Finally, we believe that DL performance on MR data prediction can be further improved, for example, by using multi-modal learning. 
%Maybe better to remove this last for example...
%
% models outperform humans
% for both Deep Learning models and humans the precision is not great, but still better than random
% suggesting that the data is noisy / difficult to predict
%
% This suggests that there is room for improvement in future work.
% Our results show that both Deep Learning models and humans outperform random predictions by a significant margin, demonstrating the predictability of MR data. However, the evaluated models do not reach human-level accuracy. This suggests that there is room for improvement in future work.
We encourage the research community to use our benchmark dataset to further investigate automatic MR data prediction.

==> sections/conclusion_old.tex <==
The Most Replayed data present a new source of insight on users' interests in online video streaming.
In this work, we focus on predicting this data using a Deep Learning (DL) model. Our efforts led to the compilation of YTMR500, a dataset comprising 500 vlog videos and their corresponding Most Replayed data.
% For this purpose, we collect YTMR500, a dataset of 500 vlog videos and their Most Replayed data, as detailed in Section \ref{section:ytmr500}.
% To predict the data, we begin with a baseline of two linear layers, and proceed to an attention-based architecture inspired by video summarization models. 
%
We begin with a baseline model of two linear layers, extending it to an attention-based architecture inspired by the video summarization model PGL-SUM \cite{PglSum}. 
As seen in Table \ref{table:ablation}, all our DL models perform significantly better than random. 
However, the application of the attention mechanism does not yield a substantial advantage over the baseline model.
%
To establish a benchmark, we conducted a crowdsourced user study involving more than 300 participants. The results (shown in Table \ref{table:user_study}) revealed that participants were not able to accurately predict the Most Replayed data.
% TODO suggesting that
% suggesting that human prior knowledge is not sufficient to understand this dataset.
%
We believe future research can further enhance the results, for instance, by incorporating multimodal inputs. We encourage the community to deploy our dataset in follow-up work.

% Eventually, we performed an ablation study on our best model. We find that the removal of the residual connection from the PGL-SUM model affects precision more substantially than removing the local or global attention modules.

==> sections/dataset_old.tex <==
\section{The YTMR500 dataset}
\label{section:ytmr500}


\begin{figure}[!ht]
\centering
\includegraphics[width=0.5\textwidth]{figures/video_grid.png}
\caption{We investigate the problem of predicting YouTube's Most Replayed data. We introduce the \emph{YTMR500} dataset, which contains 500 vlog and travel videos and the corresponding Most Replayed data.}
\label{fig:thumbs}
\end{figure}

Given a video, we investigate whether it is possible to predict which specific parts users will watch and replay. Since we are the first to tackle this problem, we cannot use pre-existing datasets. 
%
Therefore, we introduce a novel dataset of videos and annotations collected from YouTube, \emph{YTMR500} (``\textbf{Y}ou\textbf{T}ube \textbf{M}ost \textbf{R}eplayed \textbf{500}''). %, to kickstart the research on prediction and analysis of the Most Replayed data. 
The dataset consists of 500 videos, in the form of with pre-computed spatio-temporal features, and the corresponding Most Replayed data. The videos have average duration of 11.9$\pm$4.1 minutes.
%
The dataset creation process can be outlined in three main steps: (1) Data collection, (2) Feature extraction and (3) Cleanup.
% \begin{enumerate}
%     \item Data collection
%     \item Feature extraction
%     \item Cleanup
% \end{enumerate}
% \paragraph{Overview.}
\paragraph{Step 1a: Video data collection.}\label{para:ytmr50-step1a}
We retrieve videos from YouTube matching the following criteria:
\begin {enumerate*} [label=\itshape\roman*\upshape)]
\item under the Creative Commons license, \item duration from 3 to 20 minutes, and \item at least 30 thousand views. 
\end {enumerate*}
A high view count is necessary in order for YouTube to make the Most Replayed data publicly visible.
We use the search queries ``vlog'', ``trip'', ``travel'', ``visiting'' to obtain a list of videos, which are then selected to exclude those with static backgrounds or bad recording quality.
Some thumbnails of the videos in the dataset can be seen in Figure \ref{fig:thumbs}.

% \todo{Can we report some statistics here? E.g. the avg video duration, avg \# views}

\paragraph{Step 1b: Retrieval of the Most Replayed data.}
\label{para:ytmr50-step1b}
    For each of the videos in \hyperref[para:ytmr50-step1a]{Step 1a}, we download \footnote{https://github.com/Benjamin-Loison/YouTube-operational-API} the Most Replayed data, discarding those for which the data is missing.
    Concretely, the Most Replayed data consists of 100 scalars in the $[0,1]$ range, for each video. Hence, for videos of varying duration, each data point covers a different time duration.
  % Videos that resulted in errors were automatically discarded, as we aim to only have those for which the Most Replayed data is defined.
\paragraph{Step 2: Feature extraction}\label{para:ytmr50-step2}
    % After subdividing a video in segments, and use a pre-trained model to extract features for each of the video segments (not to be confused with the video shots). 
    We use a pre-trained model to extract features from the videos. The model takes as input a segment of 32 frames, which corresponds to $\sim1.1$s of video, and outputs a feature vector of 1024 dimensions. 
    This helps reduce the complexity of the input to our trained model upfront and makes the architecture compatible with any resolution and video format. It also reduces the dataset size, with our settings, by a factor of 2.7 (from 7GB to 2.6GB).
    Multiple models were taken into consideration for this step, either image-based or video-based. 
    % With image-based features, as is common in video summarization works \cite{PglSum}  CITE MORE, we would need to extract the features from a single frame in each video segment, or to average the features of multiple frames in each video segment.
    %In both cases, the image features cannot capture any relationships between the frames of the segment. 
    Image features, common in video summarization works \cite{PglSum, fajtl2019vasnet, Song2015TVSum}, cannot capture any temporal relationship between the frames of the segment.
    For this reason, we opt to use video features in our preprocessing.
    % Moreover, video features allow us to map a video segment of any duration into a single vector of fixed dimensionality.
    We choose \emph{I3D} as it is pre-trained on the extensive Kinetics-400~\cite{kay2017kinetics} and is a popular choice in the literature  \cite{doshi2022endtoend, girdhar_video_2019, Li2021BridgingTextAndVideo, mandal2019outofdistribution}. 
    Specifically, we obtain RGB features from the ``Mixed 5c'' layer of \emph{I3D}, \ie, the second-to-the-last layer, which are 1024-dimensional vectors \footnote{https://github.com/v-iashin/video\_features}.  
    Note that, for uniformity, all videos are first downsampled to 30 fps before feature extraction. 
    % Each of the features represents a segment of 32 frames of the video, which corresponds to $\sim 1.1$s.
\paragraph{Step 3: Cleanup}
    To reach the number of 500, a few excess videos are removed.
    The Most Replayed data annotations are transformed into a vector of size $100$, removing unnecessary metadata.
    % such as the constant time duration covered by each data point.
    The annotations are packaged together with the video features, having size $1024 \times T$, with $T$ proportional to video duration.
    % A H5 file with the dataset is available in our repo\footnote{https://github.com/Duico/YTMR500}. \om{Review process needs to be double blind.}
%
We will make the \emph{YTMR500} dataset available upon paper acceptance.

==> sections/discussion_old.tex <==
Based on our experiments in Section \ref{subsection:results-model}, we observe that using a more complex architecture does not induce a significant performance gain over the fully-connected baseline. Contrarily to our speculations, it seems that providing each segment with context about the full video does not improve the accuracy.
We hypothesize that the I3D video features alone provide sufficient abstraction to the fully-connected network to generate a satisfactory output from individual segments. As demonstrated by the ablation without a residual connection, hiding the input features from the fully-connected layers hinders performance, proving the importance of their role.

As shown by the users' performance in our user study in Section \ref{subsection:results-user-study}, predicting the Most Replayed data is an arduous task. One plausible explanation is that the ground truth is noisy and lacks any clear patterns with respect to the input. Upon manual analysis of several videos, we found it hard to justify the location of certain peaks in the Most Replayed data.
Another possible explanation is that video-only input does not provide enough information to resolve the problem effectively. Some peaks may be caused by interesting information in the speech, while others could result from dramatic changes in loudness. We defer to further research to incorporate multimodal inputs, particularly from audio channels and text transcripts.
% In fact, most of our models are powerful enough able to fit the training set, obtaining precision scores above 80\%, but they

==> sections/introduction_old.tex <==
Video streaming has emerged as a dominant mode of online communication, representing 73\% of all internet traffic in 2017 \footnote{Cisco VNI Forecast 2017-2022, https://newsroom.cisco.com/press-release-content?articleId=1955935}, with YouTube leading the way as the most popular platform.
% \footnote{According to statista.com, YouTube had 2.1 billion worldwide users and \$29 billion in advertising revenues in 2022. (Worldwide advertising revenues of YouTube from 2017 to 2022 (in million U.S. dollars), https://www-statista-com.tudelft.idm.oclc.org/statistics/289658/youtube-global-net-advertising-revenues/). }.
 % According to Cisco, in 2017 video streaming represented 73\% of all internet traffic, with 56.4 exabytes (EB) per month. \footnote{Cisco VNI Forecast 2017-2022,https://newsroom.cisco.com/press-release-content?articleId=1955935}
Video streaming platforms accumulate, in addition to video data, a substantial amount of metadata, pertaining to users' watching habits and interests.
Notably, in May 2022 YouTube released a new feature that shows a line chart of the most frequently replayed moments of each video, the \emph{Most Replayed} data.

In addition to aiding YouTube users during video playback, this data can serve various other potential applications, such as optimizing advertisement placement and giving feedback to content creators -- for instance, suggesting uninteresting scenes to remove.
% In both cases, publishing a video and waiting to collect the data from the first thousands of viewers is not desirable.
% For advertisements, it entails a missed revenue on the first viewers; for content creators, it causes reputational damage.
In both cases, it is desirable to predict the Most Replayed data \emph{before} publishing a video. For advertisers, it enables placing advertisements optimally from the very first views, thereby maximizing profits. For content creators, it allows cutting the video appropriately before it reaches the audience, preventing the reputational damage caused by re-uploading a video after collecting the data.

% Therefore, we attempt to train a Deep Learning (DL) model to predict the Most Replayed data.
In this work, we investigate whether it is possible to predict the Most Replayed data using Deep Learning. 
To this purpose, we collect YTMR500 (see Figure \ref{fig:thumbs}), a dataset of 500 videos and their Most Replayed data.
Subsequently, we evaluate DL models on the dataset.
We start with a simple architecture consisting of two linear layers and extend it with an attention mechanism.
Since the task is analogous to supervised video summarization, we base our extended model on the PGL-SUM architecture of Apostolidis \etal~\cite{PglSum}. 
Our adjustments consist in extracting video features instead of image features for the input videos (as detailed in Section \ref{para:ytmr50-step2}), and using a ranking loss instead of a regression loss (Section \ref{section:model}).
%
To establish a baseline against which we can compare our results, we conduct a crowdsourced user study. The participants are given 10 shots that span an entire video, and are asked to construct an estimated ranking of the shots based on the Most Replayed data. This task is a down-sized version of the one our DL model is attempting.

In this work, we make the following contributions: (1) We introduce \textit{YTMR500}, a dataset of 500 videos and the corresponding Most Replayed data, that can foster research on most replayed data predictions in videos; (2) We design a variant of the PGL-SUM~\cite{PglSum} architecture, adapted to predict the Most Replayed data for unseen videos; (3) We perform a user study to evaluate human performance on MR data prediction. Our results shows that predicting the Most Replayed data is a challenging for human annotators and that our model surpasses human performance.
%
    % OR that shows that our model surpasses human performance on this task
% \begin{itemize}
%     \item We introduce \textit{YTMR500}, a dataset of 500 videos and the corresponding Most Replayed data, that can foster research on most replayed data predictions in videos;
%     \item a variant of the PGL-SUM~\cite{PglSum} architecture, adapted to predict the Most Replayed data for unseen videos;
%     \item a user study that shows that our model surpasses human performance, as predicting the Most Replayed data is challenging for human annotators.
%     % OR that shows that our model surpasses human performance on this task
% \end{itemize}
We will make the YTMR500 dataset and all our code available upon paper publication.

==> sections/method_old.tex <==
% \section{\todo{ same as title}}
\section{Predicting the Most Replayed data in a video}
\subsection{Problem statement}
Given a sequence of segments $\bm{V}$ in a video, we design a model to learn a function $F$ that maps $\bm{V}$ into the Most Replayed (MR) data $Y$.
Specifically, the input is a sequence of 1024-dimensional video features, $\bm{v_t}$, and the output is a sequence of scores $y \in [0,1]$. Formally,
% 
% Given a sequence $\bm{V}$ of 1024-dimensional feature vectors per video segments, along with a scalar ground-truth $Y$, our model approximates a function $F$ that maps the $\bm{V}$ into the Most Replayed (MR) data $Y$.
\begin{align}
\bm{V} &=\{\bm{v_t}\}_0^T, \bm{v_t} \in \mathbb{R}^{N=1024} \\
Y      &= \{y_i\}_0^I, I=100, y_i \in [0,1] \\
F &: \bm{V} \to Y.
% \hat{Y}    &=\{\hat{y}_i\}_0^I, \hat{y}_i \in \mathbb{R}
\end{align}
% Note that each $\bm{v_t}$ is the feature vector corresponding to one segment. 
% and the y_i are ....

% Given this setup, we are interested in training a 
We want the model to determine the relative MR data of video segments when compared to one another, while we do not care about predicting the exact value of the Most Replayed data. Thus, instead of training the model using a Mean Squared Error loss, as in \cite{PglSum}, we opt for a ranking loss, namely Pytorch's \texttt{MarginRankingLoss}\footnote{https://pytorch.org/docs/2.0/generated/torch.nn.MarginRankingLoss.html}.
\begin{equation}
\label{equation:marginrankloss}
% \resizebox{.96\hsize}{!}{
        \mathcal{L}( \hat{y}_i,\hat{y}_j,s) = \max(0, {-} s_{i,j}\cdot(\hat{y}_i {-} \hat{y}_j)+\text{margin})
% }
\end{equation}

To match this setup, we construct a ranking of video segments based on the ground-truth ($y_i$) and predicted ($\hat{y}_i$) MR data scores. The \texttt{MarginRankingLoss} forces the model to predict MR scores that result in a ranking as close as possible to the ground-truth.

% The video segments can be ordered according to their MR data scores.
% We train our model by forcing it to predict MR data that results in the same segments ranking as the one obtained from the ground-truth MR data.

% We want the ranking of the $\hat{Y}$ to match that of the ground truth $Y$.
% We do not need to predict the absolute value of the Most replayed data, as our sole objective is to determine how relevant different segments are with respect to one another. Thus, instead of using a Mean Squared Error loss, as in \cite{PglSum}, we prefer to use a ranking loss, namely Pytorch's \texttt{MarginRankingLoss}\footnote{https://pytorch.org/docs/2.0/generated/torch.nn.MarginRankingLoss.html}.
% \begin{equation}
% \label{equation:marginrankloss}
% % \resizebox{.96\hsize}{!}{
%         \mathcal{L}( \hat{y}_i,\hat{y}_j,s) = \max(0, {-} s_{i,j}\cdot(\hat{y}_i {-} \hat{y}_j)+\text{margin})
% % }
% \end{equation}
% We use the \texttt{MarginRankingLoss} to enforce correct ordering of the predictions $\hat{y}_i$, with respect to the ordering of the ground truth $y_i$. 


Concretely, the loss is applied to the video segments in a pairwise fashion. In Equation~\ref{equation:marginrankloss}, the targets $s_{i,j}$ must be one of $\{1, -1, 0\}$. Here, $1$ indicates $y_i > y_j$, $-1$ indicates $y_i < y_j$, and $0$ indicates $y_i = y_j$.
To obtain these targets $s_{i,j}$, during training, we generate a comparison matrix of size $T\times T$ given by $S_{i,j} = \text{sgn}(y_i - y_j)$.
% N.B. it is necessary to mention this because S is needed below for the random sampling
Therefore the ranking of each pair of predictions $\{\hat{y}_i, \hat{y}_j\}$ is encouraged to match that of the ground truth $\{y_i, y_j\}$.
% We use the MarginRankingLoss to enforce correct ordering of the $\hat{y}_i$.
% TODO only in the ablation
%We sample a fixed number of elements from the $S_{i,j}$, so that each video will have the same contribution to the loss, independently of $T$.
%TODO experiment with a second architecture

\paragraph{Interpolation}
As mentioned in \hyperref[para:ytmr50-step1b]{Step 1b}, the Most Replayed data have a fixed length, while the number of video features varies with the duration of the videos. To use a recurrent or attention-based model, the length of the inputs and that of the outputs must match. We overcome this issue in two different ways:
\begin{enumerate}
    \item \label{case:interpolate} interpolating the ground truth to match the size of the frame features;
    \item \label{case:bin_avg} computing a binned average of the frame features, to match the size of the ground truth.
\end{enumerate}
More precisely, in Case \ref{case:interpolate} the ground truth $Y$ is interpolated from its fixed size $I=100$ into a variable size $T$. As a result, the interpolated ground truth $\widetilde{Y}$ has a different size for each of the videos, depending on the video duration.
\begin{align}
    F_1 &: \bm{V} \to \widetilde{Y}\\
    \widetilde{Y} &=\{\widetilde{y}_i\}_0^T
\end{align}
Considering that the number of frame features $T$ is always greater than $I=100$, this type of interpolation allows us to supply a larger amount of input data to the model, as compared to case 2.
Since the number of comparisons in the matrix $S$ grows quadratically with the size of the input, during training we have to randomly sample a subset of 10,000 comparisons, for each iteration and each video. Furthermore, the random sampling ensures that each video has the same contribution to the loss, independently of $T$. 
% We fixed the number of random samples to 10,000, to match Case \ref{case:bin_avg}.

In Case \ref{case:bin_avg}, we divide the frame features $\bm{V}$ in $I=100$ bins of uniform size and compute the average of the features within each bin. Therefore, the binned frame features, referred to as $\bm{\widetilde{V}}$, have a constant cardinality of $100$, regardless of the video length.
\begin{align}
    F_2 &: \bm{\widetilde{V}} \to Y\\
% Y      &= \{y_i\}_0^I, I=100, y_i \in \mathbb{R} \\
\bm{\widetilde{V}} &= \{\bm{\widetilde{v}_i}\}_0^I,~I=100,~\bm{\widetilde{v}_t} \in \mathbb{R}^{N=1024}
\end{align}
Using this strategy, the training becomes computationally easier, as there are fewer elements to be ranked.

\subsection{DL models} \label{section:model}
\begin{figure}[t]
    \centering
    % \begin{adjustbox}{width=0.8\textwidth}
    \input{model-linear}
    % \end{adjustbox}
    \caption{Our fully-connected baseline. Each of the input feature vectors is mapped to a scalar in the range $[0,1]$. We use a $50\%$ Dropout to prevent the model from overfitting the training set.}
    \label{fig:model-linear}
\end{figure}
\begin{figure*}[t]
    \centering
    \begin{adjustbox}{width=0.8\textwidth}
    \input{model-attention}
    \end{adjustbox}
    \caption{Our attention-based model architecture is inspired by PGL-SUM of Apostolidis \etal~\cite{PglSum}. The Global Attention module can capture relationships between each of the segments of the video, while the Local Attention modules focus on relationships inside a section. Ultimately, two linear layers map the vector output of the attention modules into a scalar, for each segment.}
    \label{fig:model-attention}
\end{figure*}
\paragraph{Fully connected model} As a baseline, we set up a fully-connected model, consisting of two linear layers. We also include a Dropout layer to prevent overfitting on the training set. The final layer uses a Sigmoid activation function, to coalesce the outputs into the $[0,1]$ range, similarly to the ground truth. This architecture, shown in Figure \ref{fig:model-linear}, was chosen to be similar to the final fully-connected module of the attention-based model detailed in the \hyperref[para:model-attention]{next paragraph}.
%
It is worth noting that %the input to this model is a single feature vector $\bm{v_t}$, not the full sequence $\bm{V}$. Hence, 
this architecture does not capture any temporal relationships between different segments of the video.
\paragraph{Attention-based model} \label{para:model-attention}
We investigate whether considering the temporal relationships across segments improves the MR prediction accuracy beyond our baseline.
% To enhance the accuracy beyond our baseline, we recognize the importance of considering the interactions between different feature vectors and providing context to each video segment. 
We use an attention-based model, following the architecture of PGL-SUM (Apostolidis \etal~\cite{PglSum}) as closely as possible. 
It is based on Multi-Head Attention (MAH) performed globally, \ie, for the whole duration of the video, and locally, on a number of time windows -- 4, in our setup -- obtained from a partitioning of the video.
In the global attention module, we use 8 parallel attention heads, similarly to \cite{PglSum} and to the original Transformer \cite{vaswani2017attention}. In the local attention modules we use 4 heads.
The model is shown in Figure \ref{fig:model-attention}.
% We also include Layer Normalization in between \cite{ba2016layer} the two.

\subsection{User study}

Since there exists no prior work on predicting the most replayed data in a video, there are no indications on the feasibility and difficulty of the task. We perform a user study to gain insights on how difficult predicting the most replayed data is for humans.

% \paragraph{Motivation}
% Due to 
% % the lack of previous research using the data, and 
% the introduction of a novel dataset (YTMR500, see Section \ref{section:ytmr500}), 
% it is crucial to assess human performance on the task of predicting the Most Replayed data. 
%
%\paragraph{Setup}
% We design a user study involving 30 videos randomly selected from the test set. 
Our user study contains 30 videos randomly selected from the test set. %\todo{Do we have a test set?}. 
% of one of the splits. 
For the MR data prediction, we use a different setup than for the DL model. We do this because the task performed by the DL model, \ie, constructing a ranking of 100 video segments, is too complex for human annotators. 
We simplify the task by subdividing each video in 10 shots rather than 100.
% As the complexity of the task performed by the DL model is too high for human annotators, we aim to simplify it by subdividing each video in 10 shots rather than 100. 
% As the new 10-d ground truth corresponding to each shot, we use the average of the underlying 100-d ground truths.
To match this number of shots, we average the underlying 100 ground truths into 10 bins.

We do not ask users to manually fill in the Most Replayed data, to prevent the influence of biases, \eg, a bias towards continuity of the score across segments.
Instead, we show a series of side-by-side comparisons of two video segments, to guide the users towards building a ranking.
The user study is composed of the following parts:
\begin{itemize}
    \item an introduction about the purpose of the Most Replayed data;
    \item the full video, sped up to $30$s for convenience;
    \item 19 pairwise comparisons, with the addition of an attention check.
\end{itemize}
Each comparison presents participants with two video shots, sped up to $10$s, along with the instructions: 
% \begin{displayquote}
``\textit{Guess which of the two video shots has greater `Most replayed' score.}''
% \end{displayquote}
followed by the mutually exclusive options: ``Left'', ``Right'', and ``CONTROL''.
As part of the attention check, in one extra comparison, we place a video with a text overlay asking to choose the ``CONTROL'' option. Participants who fail this simple check are rejected.

The indices for the binary comparison were derived from the execution of the MergeSort algorithm \cite{knuth1998sorting} on 10 elements. 
The number of comparisons, 19, corresponds to the number of operations that the MergeSort algorithm needs to construct a total ordering.
The indices of the segments involved in the comparisons are randomly permuted for each user, so that any imbalance with the MergeSort indices is not reflected in the outcome.
% MergeSort is a popular sorting algorithm that works on the principle of divide and conquer. Essentially, starting from sublists of 2 elements, it repeatedly merges sublists to produce new sorted sublists until there is only one sublist remaining -- the sorted list.
Once we have obtained the answers to the pairwise comparisons, we construct a graph of the ordering and perform depth-first graph traversal to reconstruct a unique ranking of the segments. 

The user study was crowdsourced to approximately 300 paid workers on Amazon MTurk \cite{mturk}. %, \todo{TODO} with an average demographic distribution. 
%
% We do not collect personal information from the crowdworkers. 
Our crowdworkers population corresponds to the average demographics on Amazon MTurk, with a uniform distribution across genders, mainly comprising residents from the US and India, born between 1990 and 2000, as reported by mturk-tracker \cite{difallah2018demographics}.
%
The number of users assigned to each video was 10 to 11, which is sufficient to obtain a statistically significant result, according to Carvalho \etal~\cite{Carvalho_Dimitrov_Larson_2016how_many_crowdsourced}.
% \begin{itemize}
%     \item Impossible to solve the same task as the AI (too much data)
%     \item binary questions reduce biases, such as local continuity and chronological bias
%     \item Simplification of the task to 10 shots
%     \item MTurk hit
%     \item numbers (12 users per video) and \cite{Carvalho_Dimitrov_Larson_2016how_many_crowdsourced}, 30 videos
%     \item inter-rater agreement is low
% \end{itemize}

==> sections/related_work_old.tex <==
\subsection{Using YouTube's metadata}
Several works investigate the use of YouTube's metadata in various scopes.
% TODO examples of types
% they have no names
Schultes \etal~\cite{schultes_leaveacomment_2013} classify YouTube comments into 3 types and 10 classes, studying their correlation with like ratio, and suggesting ways to improve the order in which they are displayed. Park \etal~\cite{park_data-driven_2021} perform a user study where they track participants watching videos on YouTube, to find associations between video view duration and other known measures, such as view count, comments per view and positive/negative sentiment of comments.
Wu and Krähenbühl~\cite{wu_towards_2021}, throughout their analysis of long-form video understanding, also attempt to predict user-engagement metrics from YouTube, namely like ratio and popularity.

% Schultes \etal~\cite{schultes_leaveacomment_2013} analyze YouTube comments as a form of communication, classifying them into three types and ten classes, studying their effects on rating and suggesting ways to improve the order in which they are displayed. 
% Abu-El-Haija \etal~\cite{abuelhaija2016youtube8m} published a dataset of approximately 8 million videos, with annotations generated from YouTube's metadata, anchor text, comments, and user engagement signals.
% Malik and Tian~\cite{malik_framework_2017} build a framework for discovering YouTube videos and collecting the metadata, overcoming the limits of the API's search function.


% Schultes \etal~\cite{schultes_leaveacomment_2013} perform an analysis of YouTube comments as a form of communication. Classify comments into 3 types and 10 classes. Study the effects of comment types on rating (Likes and Dislikes). Finally, they suggest ways to improve the way comments are displayed to the users.

% Abu-El-Haija \etal~\cite{abuelhaija2016youtube8m} publish a dataset of $\sim8$ million videos, with annotations from a vocabulary of 4800 visual entities. The annotations are automatically generated from YouTube's metadata, anchor text, comments, and user engagement signals.
% Malik and Tian~\cite{malik_framework_2017} build a framework for discovering YouTube videos and collecting the metadata, overcoming the limits of the search function of the API.
% Park \etal~\cite{park_data-driven_2021}
% Wu and Krähenbühl~\cite{wu_towards_2021}, throughout their analysis of long-form video understanding, also attempt to predict user-engagement metrics from YouTube, namely the ``YouTube like ratio'' and ``YouTube popularity''.

YouTube videos, or their extracted features, are included in several publicly available datasets \cite{abuelhaija2016youtube8m, Bose_2023_WACV, GygliECCV14SumMe, kay2017kinetics, malik_framework_2017, Song2015TVSum}.
% \cite{carreira2018short} \cite{carreira2022short}
For instance, Abu-El-Haija \etal~\cite{abuelhaija2016youtube8m} compiled a dataset of roughly 8 million videos, with annotations generated from YouTube's metadata, anchor text, comments, and user engagement signals; Kay \etal~\cite{kay2017kinetics} constructed the Kinetics-400 human action video dataset by annotating approximately 300,000 videos that were obtained from YouTube; Gygli \etal~\cite{GygliECCV14SumMe} and Song \etal~\cite{Song2015TVSum} leveraged YouTube videos to establish two of the two most commonly used video summarization datasets, SumMe and TVSum.
% Malik and Tian~\cite{malik_framework_2017} build a framework for discovering YouTube videos and collecting the metadata, overcoming the limits of the API's search function.
%
% We notice that no other authors made use of YouTube's Most Replayed data in scientific research so far, making it an interesting topic to explore.
To the best of our knowledge, we are the first to make use of YouTube's Most Replayed data in scientific research.
% , given that the data is similar in nature and dimensionality to the ``importance score'' of \ref{section/supervised-video-summ}.

\subsection{Temporal action localization}
    % Dataset of spatio-temporally localized Atomic Visual Actions (AVA)~\cite{gu_ava_2018}. Expanded by AVA-Kinetics~\cite{li_ava-kinetics_2020}.
    % \\
    % Girdhar \etal~\cite{girdhar_video_2019} introduce the Video Action Transformer Network. Trained and tested on AVA.
    % \\
    % Köpüklü \etal~\cite{kopuklu_you_2021} introduce You Only Watch Once (YOWO), using both a 3D-CNN and a 2D-CNN, whose outputs are aggregated with a Channel Fusion and Attention Mechanism.
    % \cite{pan_actor-context-actor_2021}
    % also take into account indirect higher-order relations established upon multiple elements. Propose to explicitly model the Actor-Context-Actor Relation, which is the relation between two actors based on their interactions with the context. Design an ActorContext-Actor Relation Network (ACAR-Net).

% Temporal action localization refers to the task of detecting specific actions or events within untrimmed video sequences in terms of both their types and temporal extents. This involves not only identifying what action is taking place, but also locating where it starts and ends in the timeline of the video.

% For an AI model targeting this task, the input would typically be an untrimmed video sequence, that is, a video containing one or more actions embedded within it, possibly among other irrelevant content.

% The output from such a model is typically a set of action proposals. Each action proposal consists of a start and end time (representing when the action begins and ends in the video timeline), and a class label or score distribution over all action classes (identifying the type of action taking place, such as ``jumping'', ``running'', etc.) The model essentially maps from raw video data to structured information about what actions occur when in the video.

%  TODO Explain how this is connected to MR data. Later, you can say that the output is different therefore we don't use it.
The task of predicting the Most Replayed data may be reminiscent of temporal action localization. In both cases, given a raw video stream as input, the task is to assign labels to each time step in the video. 
%
% Temporal action localization refers to the task of detecting specific actions or events within a video sequence, in terms of both their types and temporal extents \cite{shi2023tridet, shou_temporal_2016, tang2023temporalmaxer, zhang2022actionformer}.
In temporal action localization, the predicted label indicates whether a time step is part of an action and the provides the action class \cite{shi2023tridet, shou_temporal_2016, tang2023temporalmaxer, zhang2022actionformer}.
%
%refers to the task of detecting specific actions or events within a video sequence, in terms of both their types and temporal extents \cite{shi2023tridet, shou_temporal_2016, tang2023temporalmaxer, zhang2022actionformer}.
%
Temporal action localization models are typically designed to output 
% The output from such a model is typically 
a set of action proposals, which consist of a start and end time (representing when the action begins and ends in the video timeline), and a class label or score distribution over all action classes (identifying the type of action taking place, such as ``jumping'', ``running'', etc.).
Since this output structure does not match that of the Most Replayed data, we cannot base our work on any of the existing temporal action localization models.

\subsection{Connection to video summarization}
\label{section/supervised-video-summ}
% Our work is deeply connected to video summarization. 
On the other hand, our task resembles the prevailing line of research in supervised video summarization that predicts a 1D ``importance score'' for each of the segments in a video \cite{apostolidis2021survey}. In fact, we also try to predict a 1D signal, the Most Replayed data, from videos.
Differently from our work, in video summarization, the importance score is fed into a handcrafted algorithm, \eg, the 0/1 knapsack, to select which shots to include in the summary \cite{apostolidis2021survey}.
% to select the shots to be included in the summary.
% Some examples include 
% TVSum \cite{Song2015TVSum},
% vsLSTM in \cite{zhang2016video},
% bilstm \cite{ji2018bilstm} encoder architecture with two LSTMs in forward and reverse direction,
% VASnet \cite{fajtl2019vasnet},
% Apostolidis \etal~\cite{PglSum} (PGL{-}SUM), who self attention TODO,
% recollected in \cite{otani2019rethinking}) 

% Wei \etal~\cite{wei_video_2018} (SASUM) use human annotated text to perform semantic attention.
The prediction of the importance score has been tackled with LSTMs \cite{ji2018bilstm, zhang2016video, ferrari_retrospective_2018} and, more recently, with attention-based models.
Some examples of the latter include VASNet, introduced by Fajtl \etal~\cite{fajtl2019vasnet}, and PGL{-}SUM, introduced by Apostolidis \etal~\cite{PglSum}.

% The two de facto standard datasets for video summarization are SumMe~\cite{GygliECCV14SumMe} and TVSum~\cite{Song2015TVSum}. In SumMe each human annotator provides a video summary, represented by a binary annotation on predefined shots, while in TVSum each annotator provides an importance score for every 2 second segment in the original video. 
In video summarization datasets, human annotators provide either a series of binary labels, that represent the inclusion of a shot in the video summary \cite{GygliECCV14SumMe}, or directly an importance score \cite{Song2015TVSum}. In both cases, the most common way to use the annotations to train an AI model is to average them into an importance score \cite{PglSum, fajtl2019vasnet, GygliECCV14SumMe}, obtaining a format that is analogous to the Most Replayed data.
% The de facto standard datasets for video summarization are SumMe~\cite{GygliECCV14SumMe} and TVSum~\cite{Song2015TVSum}. 
% In SumMe each user provides a binary label for every  representing the video summary, while TVSum contains human annotated importance scores for every 2 second segment in the original video.
% \\
% Despite their widespread use, both datasets provide very little labeled data. In fact, TVSum consists of 50 videos labeled by 20 users and SumMe of 25 videos labeled by 15 to 20 users. Considering a typical 80/20 train/test split \cite{PglSum} \cite{fajtl2019vasnet}, the number of elements in the test set are only 10 for TVSum and 5 for SumMe. This makes it difficult to evaluate the models in a statistically significant way.
% % Most works average the user-provided labels for each video during training, practically trimming the ground truth data even more.
% \\
% In addition to the lack of sufficient ground truth data, Otani \etal~\cite{otani2019rethinking} note that the degree of inconsistency between human annotations is very high, with a Spearman's $\rho$ of 0.204 on the ranking of video shots. The subjectivity of the annotating task is stressed in \cite{fajtl2019vasnet} and \cite{Song2015TVSum}. In the latter, the authors report a pairwise F{-}score of $\sim0.36$ computed among the human labels.
% This finding compels us to seek for an alternative evaluation standard to the human annotations.

==> sections/results_old.tex <==
\paragraph{Model training}
We use 5-fold cross validation, with an 80/20 training/test ratio. That implies, of the 500 videos, 400 are utilized for training, and 100 for testing.
To train our model we follow a similar procedure to Apostolidis \etal~\cite{PglSum} and Fajtl \etal~\cite{fajtl2019vasnet}.
We use the Adam optimizer \cite{kingma2017adam} with learning rate $lr =$ \SI{5e-5} and L2 regularization $\lambda =$ \SI{1e-5} ..
Each batch contains only one sample, which is an entire video. This explains the low learning rate. 
For the \texttt{MarginRankingLoss}, we always use a margin of $0.01$, except for when we are training on 10 shots, in which case we use a margin of $0.05$.
We train for 300 epochs, because at that point the training set accuracy reaches a plateau. Even though we commonly see other research pick the best epoch with respect to the test set \cite {PglSum} \cite{fajtl2019vasnet}, we refrain from doing that not to artificially boost our results.
% Since we do not have a training/validation/test split, but only a training/test split, 
Therefore when reporting the scores we make an average over the last 50 epochs (250 to 299) and all 5 splits.

\paragraph{Evaluation metrics}
% evaluation with precision@K from information retrieval (and a ranking metric, Kendall tau~\cite{otani2019rethinking})
To evaluate our model, a ranking correlation metric could be used, \eg, Kendall's $\tau$~\cite{kendall_1938}. However, this would penalize equally errors at the bottom and at the top of the ranking. 
Furthermore, we prioritize the global ordering rather than the exact position of each element. For instance, permutations of adjacent segments in the predicted ranking should not be heavily penalized.

Hence, we use precision@K, a metric inspired from information retrieval \cite{schutze2008introduction}. precision@K measures how many of the top K results are true positives, divided by the number of results K. Given that we do not work with binary labels, we classify the top K shots in the ground truth as positives and the rest as negatives. 
Using these labels, the metric corresponds to the proportion of the top K shots of the predicted ranking that are among the top K shots in the ground truth.
We report precision@K for K in $\{15,30,50\}$, after interpolating the total number of shots to 100, when required.
The selection of $K=15$ is inspired by the evaluation practices for video summarization in the literature \cite{apostolidis2021survey} which typically adhere to a budget of 15\% of the total duration.  
The values of $K=30$ and $K=50$ were chosen to assess precision at varying ranking depths.
% This enables a more comprehensive analysis of the performance throughout the entirety of the ranking.

In the context of the user study, given that there are only 10 shots, we use values of K in $\{1,3,5\}$. It is worth noting that precision@1 corresponds to top-1 accuracy, a metric commonly used in image classification \cite{NIPS2012_c399862d}.
\subsection{DL models}
\label{subsection:results-model}
All models are able to sufficiently fit the training set, obtaining precision@50 above $80\%$ on the test set. However, the performance at test time is only marginally better than random.
Results at test time are shown at the top of Table \ref{table:ablation}.
It is surprising that our fully-connected baseline exhibits a satisfactory performance on this task, and the gains of the more complex PGL-SUM architecture are minimal.
\subsection{User study}
\label{subsection:results-user-study}
To measure inter-rater agreement, we compute the Krippendorff's alpha \cite{krippendorff2004content} among all the users, for each video. The average alpha is $-0.017 \pm 0.009$, therefore, we conclude that the users' answers are generally not coherent with one another.

In Table \ref{table:user_study} we compare the precision@K of the users' rankings and those generated by the DL model, in the simplified scenario with 10 video segments.
The top section of the table shows the results computed on the 30 videos included in the user study, while the bottom section shows the results on the complete test set, averaged on 5 splits.
% TODO fix this imprecision
Note that for the YTMR500 test set, the standard deviation is computed between the results of the 5 splits only, not across all the videos in the test set.

We report scores for our attention-based model in two scenarios: firstly, when it is trained on the ground truth interpolated to 10 data points (``trained on 10'' in Table \ref{table:user_study}), to closely match the task given to the users; secondly, when it is trained on the complete ground truth (``trained on 100'' in Table \ref{table:user_study}), and averaged into 10 bins afterward.
Naturally, training on more data, in the ``trained on 100'' case, yields better performance.

Users are not able to perform significantly better than random on this task. 
Note that users do not undergo the same training as our DL models, which means they must base their predictions on their prior knowledge.
% \todo{"In conclusion" doesn't follow from the premises}
%In conclusion, 
From the results of our user study, we believe that predicting the Most Replayed data from video segments is a difficult task for humans.

% \todo{Qualitative evaluation here}

% \begin{itemize}
%     % \item table with different lr and different loss functions
%     % \item plot of distribution of tau scores for the different videos, random vs model
%     \item results of user study
%     \item inter rater agreement is low
%     \item comparison of AI and users
% \end{itemize}

\begin{table}[tb]
% \begin{center}
\input{table_user_study}
% \end{center}
\caption{Results of our user study compared to our best DL model.
Users are not significantly better than random.
The DL models are always superior, and, with one exception, they perform better when trained on more data. \\
N.b. precision@$\{1,3,5\}$ are computed on rankings of 10 segments. The precision of the DL model is averaged over the last 50 epochs (250-299). Standard deviation is computed among the 30 videos for the User study test set and among the splits of a 5-fold cross validation for the YTMR500 test set.}
\label{table:user_study}
\end{table}

\subsection{Ablation study}
\label{subsection:ablation}
We perform an ablation study on the full model, to understand the contribution of each component. At the bottom of Table \ref{table:ablation} we report the scores for our model without local attention, without global attention and without the residual connection. We only display Case \ref{case:interpolate} of the interpolation, since the two cases are almost identical in performance.

We discover that the removal of global or local attention does not heavily impact performance, contrary to the removal of the residual connection (shown in Figure \ref{fig:model-attention}). Therefore, we deduce that the crucial part of the learning is occurring on the input frame features, within the fully-connected layers at the end of the pipeline.

% We also experiment with ...
% \begin{itemize}
%     \item without local attention
%     \item with two layers of attention
%     \item with mse loss
%     \item with augmentation windows
% \end{itemize}

\begin{table}[tb]
% \begin{center}
\input{table_ablation}
% \end{center}
\caption{Results on the test set for our models, followed by some ablations. 
All DL models perform better than random.
Surprisingly, the gains of the more complex PGL-SUM architecture are minimal, suggesting that attention between the segments is not fundamental.\\
N.b. precision@$\{15,30,50\}$ are computed on rankings of 100 segments. The numbers 1 and 2 refer to the type of interpolation: Case \ref{case:interpolate} is when the ground truth is interpolated, and Case \ref{case:bin_avg} when the frame features are averaged.}
\label{table:ablation}
\end{table}


\subsection{Discussion}
\label{subsection:discussion}

Based on our experiments in Section \ref{subsection:results-model}, we observe that using a more complex architecture does not induce a significant performance gain over the fully-connected baseline. Contrarily to our speculations, it seems that providing each segment with context about the full video does not improve the accuracy.
We hypothesize that the I3D video features alone provide sufficient abstraction to the fully-connected network to generate a satisfactory output from individual segments. As demonstrated by the ablation without a residual connection, hiding the input features from the fully-connected layers hinders performance, proving the importance of their role.

As shown by the users' performance in our user study in Section \ref{subsection:results-user-study}, predicting the Most Replayed data is an arduous task. One plausible explanation is that the ground truth is noisy and lacks any clear patterns with respect to the input. Upon manual analysis of several videos, we found it hard to justify the location of certain peaks in the Most Replayed data.
Another possible explanation is that video-only input does not provide enough information to resolve the problem effectively. Some peaks may be caused by interesting information in the speech, while others could result from dramatic changes in loudness. We defer to further research to incorporate multimodal inputs, particularly from audio channels and text transcripts.
% In fact, most of our models are powerful enough able to fit the training set, obtaining precision scores above 80\%, but they

==> table.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}
